On a Matrix Ensemble for Arbitrary Complex Quantum Systems

We present a comprehensive analytical study of a variation of the eigenvector ensemble initially proposed by Deutsch for the foundations of the Eigenstate Thermalization Hypothesis (ETH). This ensemble, called the $C$-ensemble, incorporates additional system-dependent information, enabling the study of complex quantum systems beyond the universal predictions of Random Matrix Theory (RMT). Specifically, we focus on how system-specific details influence late-time behavior in correlation functions, such as the spectral form factor, and how explicit Hamiltonian corrections not captured by RMT can be included. We demonstrate the consistency of this ensemble with respect to the universal (Haar) results by showing that it defines a unitary 1-design for arbitrary systems and for strongly chaotic systems it becomes an approximated 2-design. Universal expressions for two- and four-point ensemble-averaged correlation functions are derived, revealing how system-dependent information is spectrally decoupled. Furthermore, we show that for small energy windows, the correlation functions defined by this ensemble reduce to the predictions made by the ETH.

==> Chapters/Introduction.tex <==
\chapter{Introduction}

In the second half of the past century Wigner \cite{Wigner_Bordered-matrix_1955} in his seminal work introduced to physics what is called now days Random matrix theory (RMT) as a model for the structure of eigenvectors in complex nuclei. Since then RMT and more broadly, matrix ensembles, have become an unifying approach in physics \cite{efetov_random_2005,zyczkowski_induced_2001,iyoda_scrambling_2018,Saad/Jt_gravity_matter/2019,kostov_conformal_1999}. \par 

Perhaps one of the most important achievement of this framework dates back in the quantum chaos/semi-classical community \cite{hakee} -- where the question of how quantum systems with classical chaotic counterparts would look like -- and is the formulation of Bohigas-Gianoni-Schimt  (BGS) conjecture  \cite{bohigas-gianoni-schimt-tabor/1984}: those systems would exhibit the same universal spectral fluctuations given by an RMT Gaussian-ensemble of the proper symmetry class. Although the BSC-conjecture refers only to quantum systems with classical-analog, a wealth numerical simulation on spin-less fermions \cite{santos_onset_2010}, hard-core bosons \cite{santos_onset_2010}, spin-1/2 chains \cite{gubin_quantum_2012} and Bose-Hubbard type models \cite{parra-murillo_two-band_2013} and references therein, $``$extrapolated$"$ RMT spectral-observables like number variance and spacing-distributions \cite{dyson_statistical_1_1962} to generic many-body quantum systems has a criteria to distinguish chaotic from integrable phases, see \cite{hakee}. However, despite its widely application, RMT-spectral observable are a weak-criteria to a precise definition of what we mean by a quantum many-body chaotic system because energy eigenvalues are basis-independent data and therefore agnostic to the local physics stored in the concrete basis representation of the Hamiltonian.
 
Nowadays a further strong probe for the expected chaotic behaviors in complex many-body systems, provided by the trade off between quantum chaos and quantum information ideas \cite{Yoshida/Chaos_design/2017,Cotler/spectral_decoupling/2020,Cotler/Chaos_complexity_matrices/2018}, is the apparently universal late time behavior of correlation functions between local operators. An illustrating example of this universality is provided by two-point self correlation functions. For instance let $W$ be some highly local, then, at late times one expects approximately equalities as $\braket{e^{it H}W(t)e^{-it H}W}-\braket{W}\braket{W}\approx 0$, where the average is taken over the maximally mixed state. It is instructive to think how this connected to disconnected transition happens. For unitary chaotic quantum theories, the role of the Hamiltonian time evolution $e^{-itH}$ is to progressively mix the local operator $W$ to a non local one. For late times, this mixing becomes so strong\footnote{This is clear from the Backer-Campbell-Hausdorff formula where for late times the contribution of high commutators is relevant, i.e $e^{itH}We^{-itH}=W+it[H,W]+2!^{-1}(it)^{2}[H,[H,W]]+...$} that one is tempted to replace the Hamiltonian time evolution with a random uniformly sampled unitary without ``making many mistakes"\footnote{In particular there is a well known argument presented by M.~Berry for why the Hamiltonian time evolution can be never mirror a Haar random unitary one, and therefore is only (not a very strong) approximation of the later.}. Averaging over uniform distributed unitaries, although explains the late time expected chaotic behavior, do not give any insight on how such correlations arrived at late times in first place.
 
Chaos, in the classical (Liouville) sense defined by lack of integrals of motion, is closely related to ergodicity. Which turns into a rigorous basis to justify classical statistical mechanics in closed systems. This relationship between the origin of classical statistical mechanics in terms of non-Liuville integrable systems suggest a way in which quantum chaos could be defined, by understanding the principles of quantum statistical mechanics. Von Neumann´s quantum ergodic theorem \cite{goldstein_normal_2010}, was the first and rigorously proven result showing where, itself, the mathematical structure of a quantum-theory can yields an micro-canonical description. After Von Neumman, despite its significance, the problem about the principles of quantum statistical mechanics in closed systems saw little attention. It was not until the pioneering works of Sredenicki \cite{srednicki_chaos_1994} and Deutsch \cite{deutsch_quantum_1991} who develop the eigenstate thermalization hypothesis (ETH) \cite{Foini/Eth_OTOC/2022,Pappalardi/free_eth/2022} where statistical mechanics emerges from arguments of quantum chaos and RMT respectively that the topic would make significant progress.
 
In this thesis we present a matrix model, which we call the $C$-ensemble, constructed based on previous ideas by Deutsch's on the foundations of the ETH. We will interpret the ensemble as the equivalence class of $d!$ permutation matrices up to local phases which diagonalize a fixed given Hamiltonian $H$ on a $d$ dimensional Hilbert space. The versatility of the ensemble, due to the explicit dependence on the chosen Hamiltonian, make of it an ideal scenario to study probes on chaos in arbitrary quantum systems.

An outline of the thesis is the following:

\begin{itemize}
    \item In Chapter \ref{section:C_ensemble} we define and motivate the $C$-ensemble. Additionally, we introduce the concept of an spectral decoupled ensemble as a feature to explain universality in correlation functions.
    
    \item In Chapter \ref{Chapter:two_points} we use the $C$-ensemble to evaluate arbitrary (finite and infinite temperature) two-point correlation functions. Additionally we make comments about the relation of the $C$-ensemble with the ETH.
    
    \item In chapter \ref{Chapter_chaos} we explicitly evaluate $C$-ensemble averaged four-point out-time ordered correlation functions. Additionally we explore the complexity to build the $C$-ensemble.
    
    \item In Chapter \ref{summary_outlook} we give a short resume of the most important results and also present some ongoing future research.
    
    \item All the appendices contains original work on various formulas and derivations which support the main text.
    
\end{itemize}


